Integer round-up property for the chromatic number of some h-perfect graphs

A graph is h-perfect if its stable set polytope can be completely described by non-negativity, clique and odd-hole constraints. It is t-perfect if it furthermore has no clique of size 4. For every graph $G$ and every $c\in\mathbb{Z}_{+}^{V(G)}$, the weighted chromatic number of $(G,c)$ is the minimum cardinality of a multi-set $\mathcal{F}$ of stable sets of $G$ such that every $v\in V(G)$ belongs to at least $c_v$ members of $\mathcal{F}$. We prove that every h-perfect line-graph and every t-perfect claw-free graph $G$ has the integer round-up property for the chromatic number: for every non-negative integer weight $c$ on the vertices of $G$, the weighted chromatic number of $(G,c)$ can be obtained by rounding up its fractional relaxation. In other words, the stable set polytope of $G$ has the integer decomposition property. Our results imply the existence of a polynomial-time algorithm which computes the weighted chromatic number of t-perfect claw-free graphs and h-perfect line-graphs. Finally, they yield a new case of a conjecture of Goldberg and Seymour on edge-colorings.

==> hperf.tex <==
The purpose of this section is to prove theorem 1. We start with a reformulation of our result in terms of edge-coloring of graphs and explain how it fits into the context of previous results of Bruhn and Stein. Our theorem actually is a corollary of a slightly stronger coloring result that we prove in the second part of the section.

\subsection{Reducing to an edge-coloring problem}

Let $G$ be a graph. The line graph of $G$ is denoted $L(G)$ and is defined as follows: the vertex set of $L(G)$ is $\eds{G}$ and $u,v\in E(G)$ are adjacent in $L(G)$ if and only if they are incident in $G$. We say that $G$ is a line graph if there exists a graph $H$ such that $G$ is isomorphic to $L(H)$.

Cao and Nemhauser characterized the h-perfectness of $L(G)$ (among other notions of perfectness) in terms of excluded subdivisions in $G$. We need a few more definitions.

% INNER-DISJOINT DEFINITION, LENGTH OF A PATH
Let $C_5^{+}$ be the graph defined by $\vts{C_5^{+}}=\set{1,2,\ldots,5}$ and $\eds{C_5^{+}}=\set{12,23,34,45,15}$. In other words, $C_5^{+}$ corresponds to the 5-circuit to which we added a chord.
% FIGURE

A graph $H$ is a subdivision of $G$ if it is obtained by replacing every edge $e$ with a path $P_e$ joining the ends of $e$, such that the paths $P_e$ ($e\in\eds{G}$) are pairwise-inner-disjoint. Furthermore, it is a totally odd subdivision if each $P_e$ has odd length

A totally odd subdivision of $C_5^{+}$ is said to be an odd-$C_5^{+}$. Now, a graph $G$ is odd-$C_5^{+}$-free if it does not have a subgraph isomorphic to an odd-$C_5^{+}$.

\begin{thm}[Cao, Nemhauser]
Let $G$ be a graph. The following statements are equivalent:
\begin{itemize}
\item [i)] $L(G)$ is h-perfect,
\item [ii)] $G$ is \cfpfree.
\end{itemize}
\end{thm}

Hence, coloring the vertices of an h-perfect line graph corresponds to color the edges of a \cfpfree graph. Let us recall the basic terminology of edge-coloring. 

A matching of a graph $G$ is a set of pairwise non-incident edges of $G$. A $k$-edge-coloring of $G$ is a set of $k$ pairwise-disjoint matchings of $G$ whose union is $\eds{G}$. We say that $G$ is $k$-edge-colorable if it admits a $k$-edge-coloring.
The chromatic index of $G$, denoted $\chi'(G)$, is the smallest integer $k$ such that $G$ has a $k$-edge-coloring. In particular, $\chi(L(G))=\chi'(G)$. 
The fractional chromatic index of $G$, denoted $\chi_f'(G)$, is defined as the fractional chromatic number of $L(G)$: $\chi_f'(G)=\chi_f(L(G)$.

Using the above characterization of Cao and Nemhauser, Bruhn and Stein proved the round-up property for h-perfect line graphs in the unweighted case. Let us state their result in terms of edge-colorings:

\begin{thm}[Bruhn, Stein]
Every \cpfree graph $G$ satisfies $\chi'(G)=\ceil{\chi'_f(G)}$.
\end{thm}

Now, let us see how a problem of weighted coloring can be formulated as a edge-coloring problem. 
Let $G$ be a graph and $c\in\zset_+^{\vts{G}}$. 
It is straightforward to check that 





% EST-CE QUE CA FAIT PAS UN PEU PERSONNEL ET PAS ASSEZ QUE MATHS ?
%We mentioned in the introduction that Bruhn and Stein proved the unweighted case of theorem 1. Let us recall how they proceeded: they first showed that \cfpfree graphs with maximum degree at most 3 are 3-edge-colorable using a local recoloring technique. Using the characterization of Cao and Nemhauser, this is equivalent to state that t-perfect line graphs are 3-colorable. 
%From there on, they obtained the (unweighted) round-up property by applying the following lemma of Seb\H{o} (whose proof can also be found in REF): 
%
%% CHECK IF IT IS TRUE
%\begin{lem}[Seb\H{o}]
%Let $\mathcal{G}$ be a class of h-perfect graphs. If every triangle free t-perfect graph of $\mathcal{G}$ is 3-colorable, then every graph $G$ of $\mathcal{G}$ satisfies: $\chi(G)=\ceil{\chi(G)}$.
%\end{lem}



Our proof of the weighted case does not use Seb\H{o}'s lemma and entirely relies on edge-colorings.  The first step is reformulate the statement in terms of edge-colorings using theorem REF.















%We mentioned in the introduction that Bruhn and Stein proved the unweighted case of theorem 1:
%

%
%
%
%
%



Bruhn and Stein proved the unweighted case of theorem 1:

\begin{thm}
Every h-perfect line graph $G$ satisfies: $\chi(G)=\ceil{\chi_f(G)}$.
\end{thm}

Their proof proceeds as follows: let $H$ be a graph such that $G=L(H)$. 







% FIGURE.

Cao and Nemhauser characterized the h-perfectness of $L(G)$ in terms of the structure of $G$. Their result was already used by Bruhn and Stein to prove the unweighted case of theorem 1:




\subsection{The proof}

 





















%\textbf{back to edges of multigraphs, Cao and Nemhauser, the proof and its consequences}









%We shall prove theorem 1 in this section.
%In REF, Bruhn and Stein prove that every t-perfect line graph is 3-colorable and gave a polynomial-time algorithm to compute an optimal coloring. Using a linear programming argument of Seb\H{o}, they extended their result to the following theorem:
%
%\begin{thm}[Bruhn, Stein]
%Every h-perfect graph $G$ satisfies: $\chi(G)=\ceil{\chi_f(G)}$.
%\end{thm}
%
%As we have seen that $\chi_f(G)\leq 3$ for every t-perfect graph $G$, the theorem above indeed generalizes their 3-coloring result.
%
%Theorem 1 shows that this rounding-equality actually holds for every weight on the vertices of $G$. Our proof is also based on re-colorings along Kempe chains but we have to care about further phenomenons which are not present for simple graphs.
%
%We first recall the basic edge-coloring terminology we need and state a slightly more general result




We actually prove a slightly stronger result 





% for multigraphs, we do not need "family" of colors: we can just consider a coloration as a a partition of G into matchings !

Let $G$ be a graph. The multiplicity $\mu_G(e)$ of an edge $e$ of $G$ is the number of edges which are parallel to $e$ (including $e$). 
If $\ecol$ is an edge-coloring of $G$, we will always
%If $\ecol$ is an edge-coloring of $G$, we will say that a matching $M\in\Lambda$ \emph{occurs at} $v\in\vts{G}$ if $v$ is incident with an element of $M$.

\begin{lem}\label{lem-precol}
Let $G$ be a graph such that $\chi'(G)>\Delta(G)$ and let $e=uv$ be a critical edge of $G$. If $\ecol$ is an optimal edge-coloring of $G-e$, then:
\begin{itemize}
\item [i)] Every matching $M\in\ecol$ either covers $u$ or $v$,
\item [ii)] There exist two $A,B\in \ecol$ such that $A$ covers $u$ and misses $v$, whereas $B$ covers $v$ and misses $u$.
\end{itemize}
\end{lem}
\begin{dem}
We first prove i): by contradiction, if there exists a color $C$ of $\ecol$ which misses $u$ and $v$, 
then we can extend $\ecol$ to an edge-coloring $\ecol'$ of $G$ by adding $e$ to $C$. Since $|\ecol|=|\ecol'|$, we have $\chi'(G)\leq \chi'(G-e)$: a contradiction with the criticality of $e$.

We now show that ii) holds. Let $\ecol_u$ (resp. $\ecol_v$) denote the set of $M\in \ecol$ covering $u$ (resp. $v$) and missing $v$ (resp. $u$). By the symmetry between $u$ and $v$, it is enough to prove that $\ecol_u\nsubseteq\ecol_v$ to conclude. Seeking a contradiction, suppose $ \ecol_u\se\ecol_v $.
Using i), we have: 
\[ \chi'(G-e)=|\ecol_u\cup\ecol_v|+\mu_{G-e} (e)=|\ecol_v|+\mu_{G-e}(e)=d_{G-e}(v) =d_{G}(v)-1. \]
Hence, $\chi'(G-e)\leq \Delta(G)-1$. But since $e$ is critical we have $\chi'(G-e)=\chi'(G)-1$. Hence $\chi'(G)\leq \Delta(G)$, which contradicts our initial assumption on $G$.
\end{dem}









Let $G$ be a graph and $M$ be a matching of $G$. A chain of $G$ is \emph{$M$-alternating} if its edges consecutively alternate between $M$ and $\eds{G}\sm M$. 

A \emph{ring} of $G$ is an induced subgraph of $G$ whose underlying simple graph is a circuit. A ring is \emph{odd} if it has an odd number of vertices.

Let $G$ be a graph, $C$ an odd ring of $G$. A $C$-matching of $G$ is a matching $M$ such that $|\eds{C}\cap M|=\dfrac{|C|-1}{2}$ and $M$ misses a (necessarily unique) vertex of $C$.


% EAR: BETWEEN TO NON-ADJACENT VERTICES
% % REMPLACER LE LEMME PAR QUELQUES PHRASES BIEN CHOISIES : CEPENDANT, LE CONSERVER POUR UNE EVENTUELLE GENERALISATION
%\begin{lem}\label{lem-switch}
%Let $G$ be a graph, $N$ a $C$-matching of $G$ and $u$ the unique vertex of $C$ missed by $N$.
%Let $M$ be a matching of $G$ covering $u$ and $K$ be the component of $u$ in $(\vts{G},M\Delta N)$.
%
%If $C$ has an edge which is not in an odd-$C_5^+$ of $G$, then the following statements hold:
%\begin{itemize}
%\item [i)] $K\cap C$ is a chain,
%\item [ii)] $ |(M\Delta K)\cap C|=|M\cap C| $.
%\end{itemize}
%
%\end{lem}

%\begin{dem}[no details]

%Since $K$ is an $M$-alternating chain, we only need to prove that $K\cap C$ is an even chain.

%Since $u$ is missed by $N$, $K$ must be a chain with $u$ as an end and it is $M$-alternating (by definition).
%Let $U$ be the component of $u$ in $K\cap C$, it is a chain itself.
%
%Suppose that $U\neq K\cap C$ and let $w\in\vts{K\cap C}\sm\vts{U}$.
%Consider the path from $u$ to $w$ in $K$. It must contain an ear of $C$, which has to be odd because $N$ covers every vertex of $C$ except $u$: a contradiction with the fact that $e$ does not belong to an odd $C_5^+$.
%
%So $K\cap C=U$ is a chain and we only need to show that it is even to prove the lemma (since $K$ is $M$-alternating). We already saw that one end-edge of $U$ is in $M$ so we have to prove that the other belongs to $N$.
%If $v\in K$ then the result is obvious, and if it is not the case we see that $K$ has to leave $C$ (after traversing $U$) on an edge of $M$, hence the preceding edge was in $N$ or $U=\set{u}$, and the conclusion follows.


%First, notice that $K$ is a chain of $G$ whose edges alternate between $M$ and $N$. Indeed, since $u$ is missed by $N$ the degree to a unique edge of $K$, which belongs to $M$.
%Hence, the connected component $U$ of $u$ in $K\cap C$ is an $M$-alternating chain itself.
%
%We first prove that $U$ is even: if $|E(U)|\geq 1$, then one if its end-edges is incident with $u$ and thus belongs to $M$. So we need only to show that the other end-edge of $U$ belongs to $N$. 
%
% as $N$ is a $C$-matching, no edge of $N\sm\eds{C}$ is incident to $C$. Therefore, if $U$ has more than one vertex












%The connected components of $K\cap C$ are sub-chains of $K$, so it suffices to prove that $K\cap C$ is connected to show i).
%
%Seeking a contradiction, let us assume that $K\cap C$ has at least two connected components. 
%Put $K=(u_1,\ldots,u_k)$, where $u_1=u$, $k\geq 2$ and let $H$ be the component of $u$ in $K\cap C$.
%Now, let $i$ be the largest index such that $u_i\in H$ and $j$ the smallest index such that $u_j$ belongs to $K\cap C$ but not to $H$. 
%Consider the subchain $Q=(u_i,\ldots,u_j)$ of $K$. 
%By definition of $i$ and $j$, the chain $Q$ is non-empty, edge-disjoint from $C$ and its inner vertices (if any) do not belong to $C$.
%So $Q$ is an ear of $C$. We now prove that $Q$ is odd: this contradicts the assumption of the lemma, since $Q+C$ is an odd $C_5^+$ of $G$ containing every edge of $C$.
%As the edges of $Q$ alternate between $M$ and $N$, it suffices to show that the (not necessarily distinct) edges $e_i:=u_iu_{i+1}$ and $e_j:=u_{j-1}u_j$ which are the ends of $Q$.
%As $N$ is a $C$-matching of $G$, both $e_i$ and $e_j$ must belong to $N$. Therefore, $Q$ is odd.
%
%Now we prove ii). Since $K\cap C$ is an $M$-alternating chain, it suffices to prove that $K\cap C$ is odd.


%\end{dem}



% FAIRE UN PETIT RAPPEL SUR LES SWITCH DE COULEURS, TOUT CA...

Let $G$ be a graph. If $F\se\eds{G}$, let $\psbg{G}{F}$ denote the graph $(\vts{G},F)$.

We will often use the following classic lemma. 

\begin{lem}
Let $G$ be a graph, $\ecol$ be an edge-coloring of $G$ and $A,B$ be distinct elements of $\ecol$.

If $K$ is a connected component of $\psbg{G}{A\Delta B}$, then $ (\ecol\sm\set{A,B})\cup\set{A\Delta \eds{K},B\Delta \eds{K} } $ is an edge-coloring of $G$ which uses the same number of colors as $\ecol$. We will denote it by $\ecol^{K}$.
\end{lem}

Our main result is as follows:

\begin{thm}\label{thm-main}
Let $G$ be a graph such that $\chi'(G)>\Delta(G)$.
If $e$ is a critical edge of $G$, then one of the following statements holds:
\begin{itemize}
\item [i)] $e$ is contained in an odd-$C_5^+$ of $G$,
\item [ii)] $e$ is contained in an odd ring $R$ of $G$ such that:  
\[ |\eds{R}|= (\chi'(G)-1)r+1, \]
where $r=\dfrac{|\vts{R}|-1}{2}$. 
\end{itemize}
\end{thm}
% Don't worry about induced/chord etc.. We just have to tell clearly what we mean by it in multigraphs




\begin{dem}
Let us assume that $e$ is not contained in an odd-$C_5^+$ of $G$. We will prove ii). 
Let $u$ and $v$ be the ends of $e$, $H:=G-e$ and $\ecol$ be an optimal edge-coloring of $H$. Notice that we are under the assumptions of \myref{lem-precol}.
By its second point, there exist distinct matchings $A,B\in\ecol$ such that $A$ covers $u$ and misses $v$, whereas $B$ covers $v$ and misses $u$.

Consider the connected component $P$ of $u$ in the graph $\psbg{H}{A\Delta B}$. It is either a chain or a circuit, but $B$ misses $u$ so it must be a chain.
% The length of $P$ is even since it alternates between the two matchings $A$ and $B$ and ends with both $A$ and $B$.
% PBM : J'AI OUBLIE D'EXPLIQUER POURQUOI P CONTIENT V
If $v\notin\vts{P}$, then $(\ecol\sm\set{A,B})
\cup\set{A\Delta \eds{P},B\Delta\eds{P}}$ is an optimal edge-coloring of $G$ in which $e$ is not incident with the color class $A\Delta\eds{P}$. It can therefore be extended in an edge-coloring of $G$ with $\chi'(G-e)$ colors: a contradiction with the criticality of $e$.
Hence $P$ is a $uv$-chain and the graph $L:=P+e$ is an odd circuit of $G$. It is also induced: if $f$ is a chord of $L$, then $L+f$ forms an odd-$C_5^+$ containing $e$, which contradicts our initial assumption on $e$.  
Hence $L$ is contained in an odd ring $R$ of $G$. Let $r=(|R|-1)/2$. We claim that:
\begin{center}
\emph{$R$ contains exactly $r$ edges of each color $M$ of $\ecol$.}
\end{center}
Let us immediately show how this statement allows us to end the proof of the theorem: every edge of $R$ except $e$ belongs to one of the color classes of $\ecol$ and these are disjoint. 
Thus, the claim implies $|E(R)|=|\ecol| r+1=\chi'(G-e)\cdot r+1$, and the equality of the theorem follows from $\chi'(G-e)=\chi'(G)-1$, which holds because $e$ is critical.

We now turn to the proof of the claim above.
Let $M\in\ecol$. 
%We show that $|M\cap\eds{R}|=r$.
If $M$ is either $A$ or $B$, then $M$ has $r$ edges in $R$ because $|\vts{L}|=|\vts{R}|=2r+1$ and the edges of $P$ alternate  between $A$ and $B$.
So let us henceforth assume that $M\notin\set{A,B}$. 
% I SHOULD MAKE THE NOTATIONS COMPATIBLE: JE NE DEVRAIS PAS AVOIR A CHERCHER LE LIEN !! 

Using the symmetry between $u$ and $v$, we may assume (without loss of generality) that $M$ covers $u$.
Let $K$ be the component of $u$ in $\psbg{G}{M\Delta B}$. The graph $K$ is a chain since $B$ is an $R$-matching of $G$ which misses $u$. 
We claim that:
\begin{center}
\emph{the graph $K\cap R$ is an even chain.}
\end{center}
% DEFINIR PROPREMENT OREILLE
Indeed, if $K\cap R$ has more than one connected component then $K$ contains an ear $P'$ of $L$ with both  its end-edges in $M$. Hence $P'$ is an odd ear of $L$ (the edges of $K$ alternates between $M$ and $B$) and $L+P'$ forms an odd-$C_5^{+}$ of $G$ containing $e$: a contradiction. So $K\cap R$ is a chain. 
Now, $B$ is an $R$-matching so the end of $K\cap R$ other than $u$ (if it exists) must be covered by $B$ in $K\cap R$. Therefore $K\cap R$ has even length and this ends the proof of the claim above. It follows that :
 \[ |M'\cap \eds{R}|=|M\cap \eds{R}|, \]
where $M':=M\Delta K$.


%Recalling that $e$ does not belong to an odd-$C_5^+$, we may apply \myref{lem-switch} to show that the matching $M':=M\Delta K$ satisfies $|M'\cap R|=|M\cap R|$.
 
We now prove that $M'\cap R$ has $r$ edges in $R$.

Let $B'=B\Delta \eds{K}$  and $\ecol'=\ecol\sm\set{M,B}\cup\set{M',B'}$. Using lemma 3, we have that $\ecol'$ is an edge-coloring of $G-e$ with $|\ecol|=\chi'(G-e)$ colors and that $M'$ misses $u$. So $M'$ must cover $v$:  we could otherwise extend $\ecol'$ to an edge-coloring of $G$ by adding $e$ to $M'$, which would contradict $\chi'(G-e)<\chi'(G)$.

Let $K'$ be the component of $v$ in $\psbg{G}{M'\Delta A}$. By construction, $A$ is an $R$-matching of $G$ which misses $v$. 
Hence, we can repeat the argument of the claim above to show that $Q:=K'\cap R$ is a chain.
If $u\notin K'$, then let $M''=M\cap \eds{K'}$, $A'=A\cap \eds{K'}$ and $\ecol''=\ecol'\sm\set{M',A}\cup\set{M'',A'}$. 
As above, we apply lemma 3 to show that  $\ecol''$ is an edge-coloring of $G-e$ which uses $\chi'(G-e)$ colors. However, no edge of $M''$ is incident with $e$. It follows that $\ecol''$ can be extended to an edge-coloring of $G$ by adding $e$ to $M''$, which again contradicts $\chi'(G-e)<\chi'(G)$.

Hence, $u$ must belong to $K'$. Since $uv\notin M'$  (because $M'$ misses $u$), the only way for $Q$ to be a chain is that it coincides with the underlying simple graph of $R-e$. Therefore $|M'\cap R|=|M'\cap Q|=r$, because $Q$ is $M$-alternating and of even length.


\end{dem}

A graph $G$ is rounding-critical if $\chi'(G)>\kappa(G)$ and $\chi'(G-e)=\kappa(G-e)$ for every $e\in\eds{G}$.

For every graph $H$, let $\kappa(H)=\ceil{\chi'_f(H)}$. It is an easy exercise to show that $\kappa(H_1)\leq \kappa(H_2)$ whenever $H_1$ is a subgraph of $H_2$.

\begin{thm}
Let $G$ be a rounding-critical graph.
\end{thm}
\begin{dem}
%[of theorem \ref{thm-rc}]
Let $G$ be a rounding-critical graph. If $\eds{G}=\vn$, then the result is trivial. So let us assume that $|\eds{G}|\geq 1$ and let $e\in\eds{G}$. The edge $e$ is obviously critical, hence:
\[ \kappa(G-e)=\chi'(G-e)=\chi'(G)-1\geq \kappa(G)\geq\kappa(G-e). \]
So the inequalities above are equalities. In particular: $\kappa(G-e)=\kappa(G)$. 

Seeking a contradiction, suppose that $e$ does not belong to an odd-$C_5^{+}$. By theorem \myrefwp{thm-main}, there exists an odd ring $R$ of $G$ such that $|E(R)|=(\chi'(G-e))r+1$, where $r=(|R|-1)/2$. Hence:
\[ \kappa(G-e)=\kappa(G)\geq \dfrac{|E(R)|}{r}=\chi'(G-e)+\dfrac{1}{r}>\chi'(G-e), \]
which contradicts $\chi'(G-e)=\kappa(G-e)$.

\end{dem}

The following corollary is a straightforward consequence of theorem 2.

\begin{thm}
If $G$ is a graph without an odd-$C_5^{+}$, then $\chi'(H)=\kappa(H)$.
\end{thm}



%\section{proofs of theorem 1 and corollaries}
%
%
%\begin{dem}[of theorem 1]
%If $.\chi'(G)\leq \Delta(G)$ then we're done, otherwise:
%Let $e$ be a critical edge of $G$ which does not belong to an odd $C_5^+$.
%By the preceding theorem, there exists an odd ring $R$ such that 
%\[ \chi'(G)=\dfrac{2|E(R)|}{|R|-1}+1-\dfrac{2}{|R|-1}. \]
%Since the last term is at most 1, we have $\chi'(G)\leq \Gamma(G)+1\leq \chi_f(G)+1$.
%\end{dem}
%
%% SO WE WILL PROVE THAT H-PERFECT RELATED RESULT WITH THE ABOVE COROLLARY INSTEAD
%
%% REMARQUER QUE CHI'=CHI'^ast arrondi n'est pas héréditaire !! (Petersen + une feuille)
%By commodity, we put $\kappa(G)=\ceil{\chi'_f(G)}$ for every graph $G$.
%
%\begin{dem}[of theorem 2]
%Let $G$ be an rounding-critical graph. It is clear that $|\eds{G}|>0$. Let $e\in\eds{G}$.
%By definition $\chi'(G-e)\leq \kappa(G-e)$. Also, $\chi'(G)\leq \chi'(G-e)+1$.
%Furthermore, $\kappa(G-e)\leq \kappa(G)$. Hence:
%\[ \chi'(G-e)+1\geq \chi'(G)\geq \kappa(G)+1\geq\kappa(G-e)+1
%\geq \chi'(G-e)+1. \]
%So all the terms of the inequality above are equal. In particular, $\kappa(G-e)=\kappa(G)$ and $\chi'(G-e)<\chi'(G)$. Hence $e$ is critical.
%Seeking a contradiction, let us suppose that $e$ does not belong to an odd-$C_5+$ of $G$. Then, by the preceding theorem we have that there is an odd ring $R$ of $G$ such that $|E(R)|=(\chi'(G)-1)r$, where $r=(|C|-1)/2$. Since $r>0$ and $\chi'(G)=\chi'(G-e)-1$, this amounts to:
%\[ |E(R)|/r=\chi'(G-e)+1/r. \]
%
%By definition, $|E(R)|/r\leq\ceil{\Gamma(G)}$. Hence $\chi'(G-e)+1/r\leq \kappa(G)=\kappa(G-e)$.
%But we have $\chi'(G-e)=\kappa(G-e)$ by assumption: a contradiction.
%
%\end{dem}
%
%\begin{dem}[of corollary 1]
%direct from theorem 2.
%\end{dem}
%
%% Note that the proof of theorem 1 gives a polynomial time algorithm which, given a graph G, either finds an odd C5+ or gives a coloring of $G$ => I have to write this algorithm somewhere. + the conjecture on Graphs with odd set complexity <= 2.
%




